On Certifying Robustness against Backdoor Attacks via Randomized Smoothing

Backdoor attack is a severe security threat to deep neural networks (DNNs). We envision that, like adversarial examples, there will be a cat-and-mouse game for backdoor attacks, i.e., new empirical defenses are developed to defend against backdoor attacks but they are soon broken by strong adaptive backdoor attacks. To prevent such cat-and-mouse game, we take the first step towards certified defenses against backdoor attacks. Specifically, in this work, we study the feasibility and effectiveness of certifying robustness against backdoor attacks using a recent technique called randomized smoothing. Randomized smoothing was originally developed to certify robustness against adversarial examples. We generalize randomized smoothing to defend against backdoor attacks. Our results show the theoretical feasibility of using randomized smoothing to certify robustness against backdoor attacks. However, we also find that existing randomized smoothing methods have limited effectiveness at defending against backdoor attacks, which highlight the needs of new theory and methods to certify robustness against backdoor attacks.

==> exp.tex <==
\section{Experiments}

\subsection{Datasets and parameters}
\myparatight{Datasets and Models}
We conduct the experiments to evaluate the proposed method on CIFAR10 \citet{krizhevsky2009learning} and ImageNet \citet{deng2009imagenet}. We use the public available pre-trained model from previous work \citet{cohen2019certified}. Specifically, the architectures for the base classifier are ResNet-110 and ResNet-50 for CIFAR10 and ImageNet, respectively. 

\myparatight{Default parameters}There are several parameters we need to study. To be specific, we need to study the parameter $k$, confidence level $\alpha$, the noise level $\sigma$, number of samples $n$ and different confidence interval estimation method. Without otherwise mentioned, we use following default parameters: $k=3$, $\alpha = 0.001$, $\sigma = 0.5$, $n=100,000$ and $\textbf{SimuEM}$. Note that we set $\eta = 10^{-5}$ in all our experiments. 

\subsection{Experimental result} 
\myparatight{Compare different $k$} Fig~\ref{different_k_cifar10_imagenet} show the result for different $k$ on CIFAR10 and ImageNet dataset. As we can see, the certified accuracy increases with the increasing of the $k$ which is intuitive and consistent with theory. 

\myparatight{Compare different $\alpha$} Fig~\ref{fig_compare_alpha_cifar10_imagenet} shows the influence of $\alpha$ on two datasets. As we can see from the result, the certified accuracy XX with the increasing of $\alpha$

\myparatight{Compare different $\sigma$}Fig~\ref{different_sigma} show the result. As we can see from the result, with the increasing of $\sigma$. 

\myparatight{Compare different $n$}To do.

\myparatight{Compare BinoCP with SimuEM}Fig~\ref{different_confidence_interval_estimation} compare \textbf{BinoCP} with $\textbf{SimuEM}$. As we can see from the result, when certified radius is small, $\textbf{SimuEM}$ is better while \textbf{BinoCP} is better when certified radius is large. The reason is that when certified radius large, the value $\underline{p_l}$ is relative large, as a result, $ 1 - \underline{p_l}$ already provides a reasonable good estimation. 

\subsubsection{Compare simultaneously interval with previous work} We consider the special case when $k=1$ and compare our method to the previous work~\citet{cohen2019certified}, with different values of $\sigma$. Figure \ref{fig_compare_cifar} and Figure \ref{fig_compare_imagenet} plot the certified accuracy of the two methods on CIFAR10 and ImageNet dataset, respectively. Observe that our method has a larger certified accuracy than~\citet{cohen2019certified} when the radius is small on both CIFAR10 and ImageNet dataset. This is because we have a better estimation of $\overline{p_{b_1}}$ than $1-\underline{p_{l}}$ when $\underline{p_{l}}$ is small. However, when the radius is large, the curves of our method become lower than those derived by~\citet{cohen2019certified}. This is due to our leverage of Bonferroni correction to simultaneously estimate the probability of each class. In this case, the confidence level for each class is $1-\frac{\alpha}{c}$, compared to $1-\alpha$ that is used to estimate only $p_{l}$ in~\citet{cohen2019certified}. A larger confidence level leads to a wider confidence interval. Thus, when the radius is large, our lower bound for $\underline{p_{l}}$ is smaller while upper bound for $\overline{p_{b_1}}$ is larger, resulting in a smaller certified accuracy.


\begin{figure*}[!t]
	% \vspace{-2mm}
	 \centering
\subfloat[CIFAR10]{\includegraphics[width=0.330\textwidth]{figs/topk/cifar10/diffk/cifar_sigma0.5_diffk.pdf}}
\subfloat[ImageNet]{\includegraphics[width=0.330\textwidth]{figs/topk/imagenet/diffk/imagenet_sigma0.5_diffk.pdf}}
	 \caption{Compare different $k$ on CIFAR10 and ImageNet dataset.}
	 \label{different_k_cifar10_imagenet}
\end{figure*}

\begin{figure*}[!t]
	% \vspace{-2mm}
	 \centering
	 \subfloat[CIFAR10]{\includegraphics[width=0.330\textwidth]{figs/topk/cifar10/diffalpha/cifar_sigma0.5_k3_alpha.pdf}}
\subfloat[ImageNet]{\includegraphics[width=0.330\textwidth]{figs/topk/imagenet/diffalpha/imagenet_sigma0.5_k3_alpha.pdf}}
	 \caption{Compare different $\alpha$ for CIFAR10 and ImageNet dataset.}
	 \label{fig_compare_alpha_cifar10_imagenet}
\end{figure*}

\begin{figure*}[!t]
	% \vspace{-2mm}
	 \centering
\subfloat[CIFAR10]{\includegraphics[width=0.330\textwidth]{figs/topk/cifar10/diffsigma/cifar_k3_diffsigma.pdf}}
\subfloat[ImageNet]{\includegraphics[width=0.330\textwidth]{figs/topk/imagenet/diffsigma/imagenet_k3_diffsigma.pdf}}
	 \caption{Compare different $\sigma$ on CIFAR10 and ImageNet dataset.}
	 \label{different_sigma}
\end{figure*}

\begin{figure*}[!t]
	% \vspace{-2mm}
	 \centering
\subfloat[CIFAR10]{\includegraphics[width=0.330\textwidth]{figs/topk/cifar10/compare/top3/cifar_compare_sigma0.5_k3.pdf}}
\subfloat[ImageNet]{\includegraphics[width=0.330\textwidth]{figs/topk/imagenet/compare/top3/imagenet_compare_sigma0.5.pdf}}
	 \caption{Compare different confidence interval estimation method on CIFAR10 and ImageNet.}
	 \label{different_confidence_interval_estimation}
\end{figure*}





